The Johnson-N\'ed\'elec FEM-BEM Coupling for magnetostatic problems in the isogeometric framework

We consider a Johnson-N\'ed\'elec FEM-BEM coupling, which is a direct and non-symmetric coupling of finite and boundary element methods, in order to solve interface problems for the magnetostatic Maxwell's equations with the magnetic vector potential ansatz. In the FEM-domain, equations may be non-linear, whereas they are exclusively linear in the BEM-part to guarantee the existence of a fundamental solution. First, the weak problem is formulated in quotient spaces to avoid resolving to a saddle point problem. Second, we establish in this setting well-posedness of the arising problem using the framework of Lipschitz and strongly monotone operators as well as a stability result for a special type of non-linearity, which is typically considered in magnetostatic applications. Then, the discretization is performed in the isogeometric context, i.e., the same type of basis functions that are used for geometry design are considered as ansatz functions for the discrete setting. In particular, NURBS are employed for geometry considerations, and B-Splines, which can be understood as a special type of NURBS, for analysis purposes. In this context, we derive a priori estimates w.r.t. h-refinement, and point out to an interesting behavior of BEM, which consists in an amelioration of the convergence rates, when a functional of the solution is evaluated in the exterior BEM-domain. This improvement may lead to a doubling of the convergence rate under certain assumptions. Finally, we end the paper with a numerical example to illustrate the theoretical results, along with a conclusion and an outlook.

==> images/solutionInt.tex <==
%LaTeX with PSTricks extensions
%%Creator: inkscape 0.92.5
%%Please note this file requires PSTricks extensions
\psset{xunit=.5pt,yunit=.5pt,runit=.5pt}
\begin{pspicture}(1094.66674805,1029.33325195)
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(542.45294868,64.65959796)
\lineto(540.49982373,64.65959796)
\lineto(540.48029248,70.53850406)
\curveto(539.11310501,70.56454573)(537.74591755,70.72079573)(536.37873008,71.00725405)
\curveto(535.01154261,71.30673321)(533.63784473,71.74944153)(532.25763643,72.33537902)
\lineto(532.25763643,75.85100393)
\curveto(533.5857614,75.01767062)(534.9269072,74.38616022)(536.28107383,73.95647273)
\curveto(537.6482613,73.53980607)(539.05451126,73.32496233)(540.49982373,73.31194149)
\lineto(540.49982373,82.21819127)
\curveto(537.62221963,82.68694126)(535.52586552,83.48121207)(534.21076138,84.60100371)
\curveto(532.90867808,85.72079535)(532.25763643,87.25725365)(532.25763643,89.2103786)
\curveto(532.25763643,91.33277438)(532.96727183,93.00595142)(534.38654263,94.22990972)
\curveto(535.80581343,95.45386802)(537.84357379,96.15699301)(540.49982373,96.33928467)
\lineto(540.49982373,100.9291283)
\lineto(542.45294868,100.9291283)
\lineto(542.45294868,96.39787842)
\curveto(543.66388615,96.34579508)(544.83576112,96.21558675)(545.96857359,96.00725343)
\curveto(547.10138606,95.81194093)(548.20815687,95.53850344)(549.28888601,95.18694095)
\lineto(549.28888601,91.76897228)
\curveto(548.20815687,92.31584727)(547.09487565,92.73902434)(545.94904234,93.0385035)
\curveto(544.81622987,93.33798266)(543.65086531,93.51376391)(542.45294868,93.56584724)
\lineto(542.45294868,85.2260037)
\curveto(545.40867777,84.77027454)(547.58315688,83.95647248)(548.97638602,82.78459751)
\curveto(550.36961515,81.61272254)(551.06622971,80.01116008)(551.06622971,77.97991013)
\curveto(551.06622971,75.77938935)(550.32404223,74.04110814)(548.83966727,72.76506651)
\curveto(547.36831314,71.50204571)(545.23940694,70.77287906)(542.45294868,70.57756656)
\closepath
\moveto(540.49982373,85.57756619)
\lineto(540.49982373,93.58537849)
\curveto(538.9894071,93.41610766)(537.83706338,92.98642017)(537.04279256,92.29631602)
\curveto(536.24852175,91.60621187)(535.85138634,90.68824314)(535.85138634,89.54240984)
\curveto(535.85138634,88.4226182)(536.21596967,87.55022239)(536.94513632,86.9252224)
\curveto(537.6873238,86.30022242)(538.8722196,85.85100368)(540.49982373,85.57756619)
\closepath
\moveto(542.45294868,81.82756628)
\lineto(542.45294868,73.37053524)
\curveto(544.10659447,73.5918894)(545.35008402,74.06063939)(546.18341733,74.77678521)
\curveto(547.02977148,75.49293102)(547.45294855,76.43694142)(547.45294855,77.60881639)
\curveto(547.45294855,78.75464969)(547.04930273,79.666108)(546.24201108,80.34319132)
\curveto(545.44774027,81.02027463)(544.18471947,81.51506629)(542.45294868,81.82756628)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(557.70685455,99.69865958)
\lineto(567.86310429,66.82756666)
\lineto(564.54279188,66.82756666)
\lineto(554.38654213,99.69865958)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(571.26154171,79.17131635)
\lineto(571.26154171,92.41350352)
\lineto(574.85529162,92.41350352)
\lineto(574.85529162,79.30803509)
\curveto(574.85529162,77.23772265)(575.25893744,75.6817331)(576.06622909,74.64006646)
\curveto(576.87352073,73.61142065)(578.0844582,73.09709775)(579.6990415,73.09709775)
\curveto(581.63914562,73.09709775)(583.16909349,73.71558732)(584.28888513,74.95256645)
\curveto(585.4216976,76.18954559)(585.98810384,77.87574346)(585.98810384,80.01116008)
\lineto(585.98810384,92.41350352)
\lineto(589.58185375,92.41350352)
\lineto(589.58185375,70.53850406)
\lineto(585.98810384,70.53850406)
\lineto(585.98810384,73.89787898)
\curveto(585.11570803,72.56975401)(584.10008305,71.5801707)(582.94122892,70.92912905)
\curveto(581.79539561,70.29110824)(580.46076023,69.97209783)(578.93732277,69.97209783)
\curveto(576.424302,69.97209783)(574.51674996,70.75334781)(573.21466666,72.31584777)
\curveto(571.91258336,73.87834773)(571.26154171,76.16350392)(571.26154171,79.17131635)
\closepath
\moveto(580.30451023,92.94084725)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(606.73029082,64.65959796)
\lineto(604.77716587,64.65959796)
\lineto(604.75763462,70.53850406)
\curveto(603.39044715,70.56454573)(602.02325969,70.72079573)(600.65607222,71.00725405)
\curveto(599.28888476,71.30673321)(597.91518688,71.74944153)(596.53497858,72.33537902)
\lineto(596.53497858,75.85100393)
\curveto(597.86310354,75.01767062)(599.20424934,74.38616022)(600.55841598,73.95647273)
\curveto(601.92560344,73.53980607)(603.33185341,73.32496233)(604.77716587,73.31194149)
\lineto(604.77716587,82.21819127)
\curveto(601.89956178,82.68694126)(599.80320766,83.48121207)(598.48810353,84.60100371)
\curveto(597.18602023,85.72079535)(596.53497858,87.25725365)(596.53497858,89.2103786)
\curveto(596.53497858,91.33277438)(597.24461398,93.00595142)(598.66388477,94.22990972)
\curveto(600.08315557,95.45386802)(602.12091594,96.15699301)(604.77716587,96.33928467)
\lineto(604.77716587,100.9291283)
\lineto(606.73029082,100.9291283)
\lineto(606.73029082,96.39787842)
\curveto(607.94122829,96.34579508)(609.11310326,96.21558675)(610.24591573,96.00725343)
\curveto(611.37872821,95.81194093)(612.48549901,95.53850344)(613.56622815,95.18694095)
\lineto(613.56622815,91.76897228)
\curveto(612.48549901,92.31584727)(611.37221779,92.73902434)(610.22638448,93.0385035)
\curveto(609.09357201,93.33798266)(607.92820746,93.51376391)(606.73029082,93.56584724)
\lineto(606.73029082,85.2260037)
\curveto(609.68601991,84.77027454)(611.86049903,83.95647248)(613.25372816,82.78459751)
\curveto(614.64695729,81.61272254)(615.34357186,80.01116008)(615.34357186,77.97991013)
\curveto(615.34357186,75.77938935)(614.60138437,74.04110814)(613.11700941,72.76506651)
\curveto(611.64565528,71.50204571)(609.51674908,70.77287906)(606.73029082,70.57756656)
\closepath
\moveto(604.77716587,85.57756619)
\lineto(604.77716587,93.58537849)
\curveto(603.26674924,93.41610766)(602.11440552,92.98642017)(601.32013471,92.29631602)
\curveto(600.52586389,91.60621187)(600.12872849,90.68824314)(600.12872849,89.54240984)
\curveto(600.12872849,88.4226182)(600.49331181,87.55022239)(601.22247846,86.9252224)
\curveto(601.96466594,86.30022242)(603.14956174,85.85100368)(604.77716587,85.57756619)
\closepath
\moveto(606.73029082,81.82756628)
\lineto(606.73029082,73.37053524)
\curveto(608.38393661,73.5918894)(609.62742617,74.06063939)(610.46075948,74.77678521)
\curveto(611.30711362,75.49293102)(611.7302907,76.43694142)(611.7302907,77.60881639)
\curveto(611.7302907,78.75464969)(611.32664487,79.666108)(610.51935323,80.34319132)
\curveto(609.72508241,81.02027463)(608.46206161,81.51506629)(606.73029082,81.82756628)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(681.1779208,54.52965691)
\curveto(683.06594158,54.12601109)(684.53729571,53.28616736)(685.59198319,52.01012572)
\curveto(686.65969149,50.73408409)(687.19354565,49.15856329)(687.19354565,47.28356334)
\curveto(687.19354565,44.40595925)(686.20396234,42.1793968)(684.22479572,40.60387601)
\curveto(682.2456291,39.02835521)(679.43312917,38.24059482)(675.78729593,38.24059482)
\curveto(674.56333763,38.24059482)(673.30031683,38.36429273)(671.99823353,38.61168856)
\curveto(670.70917106,38.84606355)(669.37453567,39.20413646)(667.99432738,39.68590728)
\lineto(667.99432738,43.49450093)
\curveto(669.08807735,42.85648012)(670.28599399,42.3747093)(671.58807729,42.04918847)
\curveto(672.89016059,41.72366765)(674.25083764,41.56090723)(675.67010843,41.56090723)
\curveto(678.14406671,41.56090723)(680.02557707,42.04918847)(681.31463954,43.02575095)
\curveto(682.61672284,44.00231342)(683.26776449,45.42158422)(683.26776449,47.28356334)
\curveto(683.26776449,49.0023133)(682.66229576,50.3434591)(681.45135829,51.30700074)
\curveto(680.25344165,52.28356322)(678.58026461,52.77184445)(676.43182716,52.77184445)
\lineto(673.03338975,52.77184445)
\lineto(673.03338975,56.01403187)
\lineto(676.58807716,56.01403187)
\curveto(678.52818128,56.01403187)(680.01255624,56.39814645)(681.04120205,57.16637559)
\curveto(682.06984786,57.94762557)(682.58417076,59.06741721)(682.58417076,60.52575051)
\curveto(682.58417076,62.02314631)(682.05031661,63.16897961)(680.9826083,63.96325042)
\curveto(679.92792083,64.77054207)(678.41099378,65.17418789)(676.43182716,65.17418789)
\curveto(675.35109803,65.17418789)(674.19224389,65.0570004)(672.95526475,64.8226254)
\curveto(671.71828562,64.58825041)(670.35760857,64.22366708)(668.8732336,63.72887543)
\lineto(668.8732336,67.24450034)
\curveto(670.3706294,67.661167)(671.77036895,67.97366699)(673.07245225,68.18200032)
\curveto(674.38755638,68.39033365)(675.62453552,68.49450031)(676.78338966,68.49450031)
\curveto(679.77818125,68.49450031)(682.14797286,67.81090658)(683.89276448,66.44371911)
\curveto(685.6375561,65.08955248)(686.50995191,63.25361502)(686.50995191,60.93590675)
\curveto(686.50995191,59.32132346)(686.04771234,57.95413599)(685.1232332,56.83434435)
\curveto(684.19875405,55.72757355)(682.88364992,54.9593444)(681.1779208,54.52965691)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(694.67401421,43.76793843)
\lineto(698.79510786,43.76793843)
\lineto(698.79510786,38.80700105)
\lineto(694.67401421,38.80700105)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(719.34198234,54.52965691)
\curveto(721.23000313,54.12601109)(722.70135726,53.28616736)(723.75604473,52.01012572)
\curveto(724.82375304,50.73408409)(725.35760719,49.15856329)(725.35760719,47.28356334)
\curveto(725.35760719,44.40595925)(724.36802388,42.1793968)(722.38885727,40.60387601)
\curveto(720.40969065,39.02835521)(717.59719072,38.24059482)(713.95135748,38.24059482)
\curveto(712.72739917,38.24059482)(711.46437837,38.36429273)(710.16229507,38.61168856)
\curveto(708.8732326,38.84606355)(707.53859722,39.20413646)(706.15838892,39.68590728)
\lineto(706.15838892,43.49450093)
\curveto(707.25213889,42.85648012)(708.45005553,42.3747093)(709.75213883,42.04918847)
\curveto(711.05422213,41.72366765)(712.41489918,41.56090723)(713.83416998,41.56090723)
\curveto(716.30812825,41.56090723)(718.18963862,42.04918847)(719.47870109,43.02575095)
\curveto(720.78078439,44.00231342)(721.43182604,45.42158422)(721.43182604,47.28356334)
\curveto(721.43182604,49.0023133)(720.8263573,50.3434591)(719.61541984,51.30700074)
\curveto(718.4175032,52.28356322)(716.74432616,52.77184445)(714.59588871,52.77184445)
\lineto(711.1974513,52.77184445)
\lineto(711.1974513,56.01403187)
\lineto(714.75213871,56.01403187)
\curveto(716.69224282,56.01403187)(718.17661779,56.39814645)(719.2052636,57.16637559)
\curveto(720.2339094,57.94762557)(720.74823231,59.06741721)(720.74823231,60.52575051)
\curveto(720.74823231,62.02314631)(720.21437815,63.16897961)(719.14666985,63.96325042)
\curveto(718.09198237,64.77054207)(716.57505533,65.17418789)(714.59588871,65.17418789)
\curveto(713.51515957,65.17418789)(712.35630543,65.0570004)(711.1193263,64.8226254)
\curveto(709.88234716,64.58825041)(708.52167011,64.22366708)(707.03729515,63.72887543)
\lineto(707.03729515,67.24450034)
\curveto(708.53469095,67.661167)(709.93443049,67.97366699)(711.23651379,68.18200032)
\curveto(712.55161793,68.39033365)(713.78859706,68.49450031)(714.9474512,68.49450031)
\curveto(717.94224279,68.49450031)(720.3120344,67.81090658)(722.05682602,66.44371911)
\curveto(723.80161765,65.08955248)(724.67401346,63.25361502)(724.67401346,60.93590675)
\curveto(724.67401346,59.32132346)(724.21177389,57.95413599)(723.28729474,56.83434435)
\curveto(722.3628156,55.72757355)(721.04771147,54.9593444)(719.34198234,54.52965691)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(751.0412003,50.64293826)
\lineto(751.0412003,48.8851258)
\lineto(734.51776321,48.8851258)
\curveto(734.67401321,46.41116753)(735.41620069,44.52314674)(736.74432566,43.22106344)
\curveto(738.08547146,41.93200097)(739.94745058,41.28746974)(742.33026302,41.28746974)
\curveto(743.71047132,41.28746974)(745.0451067,41.45674057)(746.33416917,41.79528223)
\curveto(747.63625247,42.13382389)(748.92531494,42.64163637)(750.20135657,43.31871969)
\lineto(750.20135657,39.92028227)
\curveto(748.9122941,39.37340729)(747.59067955,38.95674063)(746.23651292,38.67028231)
\curveto(744.88234629,38.38382398)(743.5086484,38.24059482)(742.11541927,38.24059482)
\curveto(738.62583603,38.24059482)(735.85890901,39.25621979)(733.81463823,41.28746974)
\curveto(731.78338828,43.31871969)(730.76776331,46.06611545)(730.76776331,49.52965703)
\curveto(730.76776331,53.11038611)(731.73130495,55.94892771)(733.65838823,58.04528182)
\curveto(735.59849235,60.15465677)(738.20916937,61.20934424)(741.49041929,61.20934424)
\curveto(744.43312755,61.20934424)(746.75734624,60.25882343)(748.46307536,58.35778181)
\curveto(750.18182532,56.46976103)(751.0412003,53.89814651)(751.0412003,50.64293826)
\closepath
\moveto(747.44745039,51.69762573)
\curveto(747.42140872,53.66377151)(746.86802332,55.23278189)(745.78729418,56.40465686)
\curveto(744.71958587,57.57653183)(743.30031508,58.16246932)(741.52948179,58.16246932)
\curveto(739.5242735,58.16246932)(737.91620063,57.59606308)(736.70526316,56.46325061)
\curveto(735.50734652,55.33043814)(734.81724237,53.7353861)(734.63495071,51.67809448)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(755.12323145,51.36559449)
\lineto(765.65057493,51.36559449)
\lineto(765.65057493,48.16246957)
\lineto(755.12323145,48.16246957)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(780.31854332,65.36950039)
\curveto(778.28729337,65.36950039)(776.75734549,64.36689625)(775.72869968,62.36168796)
\curveto(774.71307471,60.36950051)(774.20526222,57.3681985)(774.20526222,53.35778194)
\curveto(774.20526222,49.3603862)(774.71307471,46.3590842)(775.72869968,44.35387591)
\curveto(776.75734549,42.36168846)(778.28729337,41.36559474)(780.31854332,41.36559474)
\curveto(782.3628141,41.36559474)(783.89276198,42.36168846)(784.90838695,44.35387591)
\curveto(785.93703276,46.3590842)(786.45135566,49.3603862)(786.45135566,53.35778194)
\curveto(786.45135566,57.3681985)(785.93703276,60.36950051)(784.90838695,62.36168796)
\curveto(783.89276198,64.36689625)(782.3628141,65.36950039)(780.31854332,65.36950039)
\closepath
\moveto(780.31854332,68.49450031)
\curveto(783.5867724,68.49450031)(786.08026192,67.19892743)(787.79901188,64.60778166)
\curveto(789.53078267,62.02965672)(790.39666807,58.27965682)(790.39666807,53.35778194)
\curveto(790.39666807,48.44892789)(789.53078267,44.69892799)(787.79901188,42.10778222)
\curveto(786.08026192,39.52965728)(783.5867724,38.24059482)(780.31854332,38.24059482)
\curveto(777.05031423,38.24059482)(774.5503143,39.52965728)(772.81854351,42.10778222)
\curveto(771.09979355,44.69892799)(770.24041857,48.44892789)(770.24041857,53.35778194)
\curveto(770.24041857,58.27965682)(771.09979355,62.02965672)(772.81854351,64.60778166)
\curveto(774.5503143,67.19892743)(777.05031423,68.49450031)(780.31854332,68.49450031)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(798.01385538,42.12731347)
\lineto(804.45916771,42.12731347)
\lineto(804.45916771,64.37340666)
\lineto(797.44744914,62.9671567)
\lineto(797.44744914,66.56090661)
\lineto(804.42010522,67.96715657)
\lineto(808.36541762,67.96715657)
\lineto(808.36541762,42.12731347)
\lineto(814.81072996,42.12731347)
\lineto(814.81072996,38.80700105)
\lineto(798.01385538,38.80700105)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(367.09337461,67.99753428)
\curveto(365.06212466,67.99753428)(363.53217678,66.99493014)(362.50353098,64.98972185)
\curveto(361.487906,62.9975344)(360.98009351,59.99623239)(360.98009351,55.98581583)
\curveto(360.98009351,51.9884201)(361.487906,48.98711809)(362.50353098,46.9819098)
\curveto(363.53217678,44.98972235)(365.06212466,43.99362863)(367.09337461,43.99362863)
\curveto(369.13764539,43.99362863)(370.66759327,44.98972235)(371.68321825,46.9819098)
\curveto(372.71186405,48.98711809)(373.22618696,51.9884201)(373.22618696,55.98581583)
\curveto(373.22618696,59.99623239)(372.71186405,62.9975344)(371.68321825,64.98972185)
\curveto(370.66759327,66.99493014)(369.13764539,67.99753428)(367.09337461,67.99753428)
\closepath
\moveto(367.09337461,71.1225342)
\curveto(370.3616037,71.1225342)(372.85509322,69.82696132)(374.57384317,67.23581555)
\curveto(376.30561396,64.65769061)(377.17149936,60.90769071)(377.17149936,55.98581583)
\curveto(377.17149936,51.07696178)(376.30561396,47.32696188)(374.57384317,44.73581611)
\curveto(372.85509322,42.15769117)(370.3616037,40.86862871)(367.09337461,40.86862871)
\curveto(363.82514553,40.86862871)(361.32514559,42.15769117)(359.5933748,44.73581611)
\curveto(357.87462484,47.32696188)(357.01524986,51.07696178)(357.01524986,55.98581583)
\curveto(357.01524986,60.90769071)(357.87462484,64.65769061)(359.5933748,67.23581555)
\curveto(361.32514559,69.82696132)(363.82514553,71.1225342)(367.09337461,71.1225342)
\closepath
}
}
\end{pspicture}

